The Complexity of Admissibility in Omega-Regular Games

Iterated admissibility is a well-known and important concept in classical game theory, e.g. to determine rational behaviors in multi-player matrix games. As recently shown by Berwanger, this concept can be soundly extended to infinite games played on graphs with omega-regular objectives. In this paper, we study the algorithmic properties of this concept for such games. We settle the exact complexity of natural decision problems on the set of strategies that survive iterated elimination of dominated strategies. As a byproduct of our construction, we obtain automata which recognize all the possible outcomes of such strategies.

==> macrosElimstrat.tex <==
\makeatletter
%% General
\newcommand{\mmid}{\:\middle|\:}

%% Maths
\newcommand{\stratset}{\ensuremath{\mathcal{S}}}
\newcommand{\dom}[1]{\ensuremath{\succcurlyeq_{#1}}}
\newcommand{\domstr}[1]{\ensuremath{\succ_{#1}}}
\newcommand{\trdom}[1]{\ensuremath{\mathrel{\raisebox{0.75ex}{$\xrightarrow$}\hspace{-2.75ex}\succcurlyeq_{#1}}}}
\newcommand{\trdomstr}[1]{\ensuremath{\mathrel{\raisebox{0.75ex}{$\rightarrow$}\hspace{-2.75ex}\succ_{#1}}}}	\newcommand{\win}[1]{\ensuremath{\textsc{Win}_{#1}}}
\newcommand{\weight}[1]{\ensuremath{\textsc{w}_{#1}}}
\newcommand{\bad}{\ensuremath{\mathit{Bad}}}
\newcommand{\good}{\ensuremath{\mathit{Good}}}
\newcommand{\buchi}{\ensuremath{F}}
\newcommand{\cobuchi}{\ensuremath{\overline{\buchi}}}
\newcommand{\nondom}{\ensuremath{\textsc{Nd}}}
\newcommand{\runs}{\ensuremath{\mathit{Runs}}}
\newcommand{\outcome}{\ensuremath{\mathit{Out}}}
%\newcommand{\occurrence}[1]{\ensuremath{\mathit{Occ}_{#1}}}
\newcommand{\val}{\ensuremath{\mathrm{Val}}}
\newcommand{\optval}{\ensuremath{\mathrm{Pes}}}
\newcommand{\aval}{\ensuremath{\mathrm{Opt}}}
%\newcommand{\hval}[2]{\ensuremath{\widehat{\mathrm{Val}}^{#1}_{#2}}}
\newcommand{\hval}[2]{\ensuremath{\mathrm{ValR}^{#1}_{#2}}}
\newcommand{\coalition}[1]{\ensuremath{\left\langle\!\left\langle#1\right\rangle\!\right\rangle}}
%\newcommand{\ecoalition}[1]{\ensuremath{\left\langle\!\left\langle#1\right\rangle\!\right\rangle}}
%\newcommand{\acoalition}[1]{\ensuremath{\left[\!\left[#1\right]\!\right]}}
\newcommand{\globally}{\ensuremath{\square}}
\newcommand{\eventually}{\ensuremath{\diamond}}

%% Lettres fr\'equentes
%%% Fonctions d'ordre sup\'erieur
\newcommand{\m@ken@medcal}[2][\@error]{\expandafter\def\csname #1\endcsname{\ensuremath{\mathcal{#2}}}}
\newcommand{\m@kecal}{\@dblarg\m@ken@medcal}
\newcommand{\m@ken@medbb}[2][\@error]{\expandafter\def\csname #1\endcsname{{\ensuremath{\mathbb{#2}}}}}
\newcommand{\m@kebb}{\@dblarg\m@ken@medbb}
\newcommand{\m@ken@medsf}[2][\@error]{\expandafter\def\csname #1\endcsname{{\ensuremath{\mathsf{#2}}}}}
\newcommand{\m@kesf}{\@dblarg\m@ken@medsf}
%%% CALigraphiques
\m@kecal{A}
\m@kecal{B}
\m@kecal{G}
\m@kecal{H}
\m@kecal{T}
\m@kecal[lingame]{L}
\m@kecal{L} %%% Pas bien: 2 choses ont la meme typographie
\m@kecal[circuit]{C}
%%% Black-Board
\m@kebb{N}
\m@kebb{Q}
\m@kebb{Z}
%%% Sans-s\'eriF
%\m@kesf[propp]{p}
%%% Autres
\newcommand{\eps}{\varepsilon}
\newcommand{\oneto}[1]{\left\{1,\dots,#1\right\}}
\newcommand{\lattice}{\Lambda}

\def\relB{\mathrel{\blacktriangleleft}}
\def\relBb{\mathrel{\ntriangleleft}}

\def\Adam{\texttt{Adam}\xspace}
\def\Eve{\texttt{Eve}\xspace}
\def\eve{\Eve}
\def\adam{\Adam}
\def\evebis{\texttt{Loner}\xspace}
\def\adambis{\texttt{Teamer}\xspace}
\def\shortEve{\ensuremath{\exists}}
\def\shortAdam{\ensuremath{\forall}}
\def\shortEvebis{\ensuremath{\mathtt{L}}}
\def\shortAdambis{\ensuremath{\mathtt{T}}}
\def\sigmaEve{\ensuremath{{\sigma_\shortEve}}\xspace}
\def\sigmaAdam{\ensuremath{{\sigma_\shortAdam}}\xspace}
\def\QSAT{\ensuremath{\ComplexityFont{QSAT}}\xspace}
\def\EXPTIME{\ensuremath{\ComplexityFont{EXPTIME}}\xspace}
\def\NEXPTIME{\ensuremath{\ComplexityFont{NEXPTIME}}\xspace}
\def\profile{\ensuremath{\sigma_{\!\Agt}}\xspace}
\def\MP{\ensuremath{\mathtt{MP}}}
\newcommand\profileminus[1]{\ensuremath{\sigma_{-#1}}\xspace}
\newcommand\player[1]{player~$#1$\xspace}
\newcommand\visited{\ensuremath{R}}
\newcommand\lost{\lambda}
\newcommand\won{\gamma}
\newcommand\env{\textit{env}}

\def\proj{\mathsf{proj}}
\def\pathproj{\overrightarrow{\mathsf{proj}}}
\newcommand{\last}{\ensuremath{\mathrm{last}}}
\newcommand{\states}[1]{\ensuremath{\mathrm{Occ}\!\left({#1}\right)}}
\newcommand{\prestates}[1]{\ensuremath{\mathrm{Occ}^{-1}\!\left({#1}\right)}}
\def\occ{\states}
\def\stateset{\ensuremath{O}}
\newcommand{\inff}[1]{\ensuremath{\mathrm{Inf}({#1})}}
\def\ie{i.e.\xspace}
\def\newdef{\emph}
\def\Agt{\ensuremath{P}}
%\def\nBC{\ensuremath{\overline{BC}}}
\newcommand\nBC[1]{\ensuremath{\outcome(\G\setminus T^{#1})}}

\newcommand{\prefix}{\ensuremath{\olessthan}}
\newcommand{\pref}[1]{\preccurlyeq_{#1}}
%\newcommand{\Hcompatible}[1]{\ensuremath{\stackrel[\shortEve]{j}{\bowtie}}}
\newcommand{\Hcompatible}[1]{\ensuremath{\bowtie_\shortEve^{#1}}}
\newcommand{\Gcompatible}[1]{\ensuremath{\bowtie_\G^{#1}}}
\newcommand{\oneplayer}{\ComplexityFont{1PG}\xspace}
\newcommand{\twoplayer}{\ComplexityFont{2PG}\xspace}
\newcommand{\valgame}{\ensuremath{\mathsf{val}\G}\xspace}

\newcommand{\switch}[2]{\ensuremath{\left[#1\leftarrow#2\right]}}
\newcommand{\switchbis}[2]{\ensuremath{#1\left[#2\right]}}

\newcommand{\trans}[2]{\ensuremath{#1\rightarrow#2}}
%\newcommand{\trans}[2]{\ensuremath{(#1,#2)\in E}}
\newcommand{\sigmadict}{\ensuremath{\sigma^{\text{dict}}_\shortEvebis}}
\newcommand{\sigmalinear}{\ensuremath{\sigma^{\ell}_\shortEvebis}}
\newcommand{\sigmaa}{\ensuremath{\alpha}}
\newcommand{\sigmal}{\ensuremath{\sigma^\ell}}
%\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\lsem}{\ensuremath{[\mkern-3mu[}}
\newcommand{\rsem}{\ensuremath{]\mkern-3mu]}}


\tikzstyle{bigloop}+=[distance=1cm,looseness=1]
\tikzstyle{bigloop right}+=[bigloop,out=30,in=-30]
\tikzstyle{bigloop left}+=[bigloop,out=150,in=-150]
\tikzstyle{bigloop above}+=[bigloop,out=120,in=60]
\tikzstyle{bigloop below}+=[bigloop,out=-120,in=-60]
\tikzstyle{player1}=[state,shape=circle]
\tikzstyle{player2}=[state,shape=rectangle]
\tikzstyle{player3}=[state,shape=isosceles triangle,shape border rotate=90, isosceles triangle apex angle=110]
\newcommand{\train}[5][1]{%
\begin{scope}[#1]
\path[draw={#2},fill={#3}] (0,0) -- ++(1,0) arc (-225:45:1.125) -- ++(3,0) arc (-225:45:1.125) -- ++(0.5,0) -- ++(0.66,-1.66) -- ++(1.5,0) -- ++(-1.25,1.66) -- ++(0.5,0) arc (-20:20:3) -- ++(-0.5,0) -- ++(0.5,2) -- ++(-0.25,0.25) -- ++(-1.5,0) -- ++(-0.25,-0.25) -- ++(0.55,-2) -- ++(-4,0) -- ++(0,0.25) .. controls +(0.75,0.5) and +(1.5,0) .. ++(0,2.5) -- ++(-4,0) -- ++(0,-0.5) .. controls +(1,-0.5) and +(1.25,0.75) .. (0,0.33) -- cycle;
\node[anchor=center,text={#4}] at (2.125,2.25) {#5};
\end{scope}
}
\newcommand{\minitrain}[3]{\tikz{\train[scale=0.1]{black}{#1}{#2}{\Large\textbf{\textsf{#3}}}}}
\newcommand{\minirevtrain}[3]{\tikz{\train[yscale=0.1,xscale=-0.1]{black}{#1}{#2}{\Large\textbf{\textsf{#3}}}}}
\newcommand{\txttrain}[1]{\tikz{\train[scale=0.05]{#1}{#1}{#1}{}}\xspace}
\newcommand{\txtrevtrain}[1]{\tikz{\train[yscale=0.05,xscale=-0.05]{#1}{#1}{#1}{}}\xspace}
\definecolor{lipicsyellow}{rgb}{0.99,0.78,0.07}
\makeatother

%\renewcommand\emptyset\varnothing

